A Time and Space Efficient Algorithm for Contextual Linear Bandits

We consider a multi-armed bandit problem where payoffs are a linear function of an observed stochastic contextual variable. In the scenario where there exists a gap between optimal and suboptimal rewards, several algorithms have been proposed that achieve $O(\log T)$ regret after $T$ time steps. However, proposed methods either have a computation complexity per iteration that scales linearly with $T$ or achieve regrets that grow linearly with the number of contexts $|\myset{X}|$. We propose an $\epsilon$-greedy type of algorithm that solves both limitations. In particular, when contexts are variables in $\reals^d$, we prove that our algorithm has a constant computation complexity per iteration of $O(poly(d))$ and can achieve a regret of $O(poly(d) \log T)$ even when $|\myset{X}| = \Omega (2^d) $. In addition, unlike previous algorithms, its space complexity scales like $O(Kd^2)$ and does not grow with $T$.

==> bibitems.tex <==
\bibitem{langford2007epoch}
Langford, J., Zhang, T.: The epoch-greedy algorithm for contextual multi-armed bandits. Advances in Neural Information Processing Systems 20 (2007)

\bibitem{dudik2011efficient}
Dudik,M.,Hsu,D.,Kale,S.,Karampatziakis,N.,Langford,J.,Reyzin,L.,Zhang, T.: Efficient optimal learning for contextual bandits. In: UAI. (2011)

\bibitem{auer2002finite} 
Auer, P., Cesa-Bianchi, N., Fischer, P.: Finite-time analysis of the multiarmed bandit problem. Machine learning 47(2) (2002) 235Ð256

\bibitem{johnson1978}
Johnson, D., Preparata, F.: The densest hemisphere problem. Theoretical Com- puter Science 6 (1978)

\bibitem{bartlett99} 
Bartlett, P., Ben-David, S.: On the hardness of learning with neural networks. In: European Conference on Computational Learning Theory. (1999)

\bibitem{auer2002tradeoffs} 
Auer, P.: Using confidence bounds for exploitation-exploration trade-offs. Journal of Machine Learning Research 3 (2002)

\bibitem{li2010contextual}
Li, L., Chu, W., Langford, J., Schapire, R.: A contextual-bandit approach to per- sonalized news article recommendation. 
In: Proceedings of the 19th international conference on World wide web, ACM (2010) 661Ð670

\bibitem{chu2011contextual} 
Chu, W., Li, L., Reyzin, L., Schapire, R.: Contextual bandits with linear payoff functions. In: Conference on Artificial Intelligence and Statistics (AISTATS). (2011)

\bibitem{dani2008stochastic} 
Dani, V., Hayes, T., Kakade, S.: Stochastic linear optimization under bandit feedback. In: Proceedings of the 21st Annual Conference on Learning Theory (COLT). (2008)

\bibitem{rusmevichientong2008linearly} 
 Rusmevichientong, P., Tsitsiklis, J.: Linearly parameterized bandits. Mathematics of Operations Research 35(2) (2010)

\bibitem{abbasi2011improved} 
Abbasi-Yadkori, Y., Pa?l, D., Szepesva?ri, C.:	Improved algorithms for linear stochastic bandits. Advances in Neural Information Processing Systems (2011)

\bibitem{barto1998} 
 Sutton, Barto: Reinforcement learning, and introduction. Cambdrige, MIT Press (1998)
